Mid-Band 5G: A Measurement Study in Europe and US

Fifth Generation (5G) mobile networks mark a significant shift from previous generations of networks. By introducing a flexible design, 5G networks support highly diverse application requirements. Currently, the landscape of previous measurement studies does not shed light on 5G network configuration and the inherent implications to application performance. In this paper, we precisely fill this gap and report our in-depth multi-country measurement study on 5G deployed at mid-bands. This is the common playground for U.S. and European carriers. Our findings reveal key aspects on how carriers configure their network, including spectrum utilization, frame configuration, resource allocation and their implication on the application performance.

==> 10-conclude.tex <==

\section{Conclusion}
\label{s:conclude}

We have presented, to the best of our knowledge, the  first large-scale cross-country, comparative 5G measurement study of 5G mid-band deployments in four major European countries and the US, covering 9 European 5G operators and 3 major US 5G operators.  Through \emph{in-depth} 
\emph{cross-layer} data analysis,  we have uncovered the key 5G mid-band channels and configuration parameters employed by various operators in these countries, 
and identified the major factors that impact the observed 5G performance both from the network 
perspective  as well as the application perspective. Our results show the complexity and intricacies of 
5G networks --- how various 5G configurations and dynamic parameters, such as channel bandwidth, resource blocks, channel conditions, modulation order, coding rate, MIMO, carrier aggregation, etc.,  influence the observed 5G network and application performance. Our study can aid 5G operators in better configuring and optimizing their 5G networks, and guide users, application developers and cloud providers in making carrier selection, application tuning and server placement choices. 
Our study also opens up new avenues for exploration such as artificial intelligence and machine learning (AI/ML) in 5G networks, and provides invaluable insights into the design of next-generation 
mobile networks and applications.
Lastly,  we note that our datasets, analyses and results (e.g., roaming configurations and their impact on application performance) are richer and more expansive than what we have reported in this paper. Due to space limitation, we are not able to include them here. 




 




